Automatic Calibration of Multiple 3D LiDARs in Urban Environments

Multiple LiDARs have progressively emerged on autonomous vehicles for rendering a wide field of view and dense measurements. However, the lack of precise calibration negatively affects their potential applications in localization and perception systems. In this paper, we propose a novel system that enables automatic multi-LiDAR calibration without any calibration target, prior environmental information, and initial values of the extrinsic parameters. Our approach starts with a hand-eye calibration for automatic initialization by aligning the estimated motions of each sensor. The resulting parameters are then refined with an appearance-based method by minimizing a cost function constructed from point-plane correspondences. Experimental results on simulated and real-world data sets demonstrate the reliability and accuracy of our calibration approach. The proposed approach can calibrate a multi-LiDAR system with the rotation and translation errors less than 0.04 [rad] and 0.1 [m] respectively for a mobile platform.

==> contribution.tex <==
\section{New Contribution}
\label{sec.contribution}

\subsection{Overview of the Method}
Inspired by the previous work \cite{taylor2012mutual,taylor2015motion,taylor2016motion,heng2013camodocal,segal2009generalized}, we combine with motion-based and appearance-based approaches to propose an automatic extrinsic calibration method for multi-lidar sensing system in this paper. This method takes the essential ideas used in hand-eye calibration problem to initialize the extrinsic parameters. Then when overlapping of lidars exists, further refinement is done by making use of the appearance information provided by sensors. To our best knowledge, there is no existing work focusing on motion-based multi-lidar calibration. \\

Considering that this sensing system will be mounted on autonomous vehicles, the calibration method should be friendly to non-expert users and successfully used in natural scenes, like roads and streets. To simplify the problem, we assume that several prior knowledge is known:
\begin{enumerate}
	\item The lidars are synchronized.
	\item The lidars are rigidly mounted.
	\item The lidars' intrinsic parameters are known.
	\item The measurements of lidars have a dominant ground plane.
	\item The lidars undergo a series of known and nondegenerate motion. \\
\end{enumerate}

The first assumption means that the relative transformations of lidars at each timestamp $\textbf{T}_{L_i,k}^{L_1,k-1}$ are synchronized. The second assumption ensures that the extrinsic parameters $\underset{1\leq i\leq N}{\bigcup}\{\textbf{T}_{L_i}^{L_1}\}$ are unique. The third assumption ensures that measurements of lidars are undistorted. The fourth assumption is common in outdoor environments and can be used in further appearance-based refinement. And the final assumption guarantees solvable $\textbf{R}$ and $\textbf{t}$ given by enough data.

\subsection{Contribution}
With assumptions made, the contributions of this paper include the following:
\begin{enumerate}
	\item We propose an automatic multi-lidar extrinsic calibration method that doest not require any initial guess. The method can work on sensors with/without overlapping fields of view.
	\item We present the usage of appearance-based approaches to refine the results of motion-based calibration. 
\end{enumerate}

\subsection{Algorithm}
The automatic calibration method is summarized in Algorithm \ref{alg.proposed_method}. Here we use $\textbf{R}, \textbf{t}$ to express transformation instead of $\textbf{T}$. 
Similar to \cite{taylor2016motion, heng2013camodocal}, the algorithm has three steps: motion estimation (line 1-3), initialization (line 5-18), and refinement (line 19). \\

\subsubsection{Motion estimation}
To calculate the relative transformation of consecutive frames of lidars, lightweight lidar odometry and mapping (LOAM) \cite{zhang2014loam} is used. The odometry part of LOAM is a modified ICP which combines point-to-point and point-to-plane metrics. \\

\subsubsection{Initialization}
\label{subsubsec.initialization}
The function of this step is to get an good initial guess, specially, to solve equ. (\ref{equ.rotation_axes}) and (\ref{equ.ls_translation}). Regarding the rotation, a modified version of the Kabsch algorithm developed in \cite{taylor2016motion} is applied. Once the rotation matrix is known, the translation can be calculated using linear least square techniques. Starting with equ. (\ref{equ.ls_translation}), the terms can be rearranged and combined with information from each timestamps to give equ. (\ref{equ.lls}):
\begin{equation}
\begin{split}
\textbf{t}_{y}^{x} = 
\begin{bmatrix}
\textbf{R}_{x,k}^{x,k-1} - \textbf{I} \\
\textbf{R}_{x,k+1}^{x,k} - \textbf{I} \\
\cdots \\        
\end{bmatrix}^{-1}
\begin{bmatrix}
\textbf{R}_{y}^{x}\textbf{t}_{y,k}^{x,k-1} - \textbf{t}_{x,k}^{x,k-1} \\
\textbf{R}_{y}^{x}\textbf{t}_{y,k+1}^{x,k} - \textbf{t}_{x,k+1}^{x,k} \\
\cdots \\        
\end{bmatrix}\\
\end{split}
\label{equ.lls}
\end{equation}

The translation estimate is dependent highly on the accuracy of rotation matrix calculation and sensitive to noise in motion estimation. But in many instances, $\textbf{R}_{x,k}^{x,k-1} \approx \textbf{I}$ leads the left matrix approximate to $\textbf{0}$. Dividing by this matrix reduces the signal-to-noise ratio (SNR) and thus degrades the estimation. Consequently the translation estimates are less accurate than the rotation estimates \cite{taylor2016motion}. \\

In addition, due to uncertainty in motion estimation, we use random sample consensus (RANSAC) algorithm \cite{fischler1981random} to reject outliers. Please see line 9-13 or line 15-19 for detailed steps.\\

\subsubsection{Refinement}
In this step, we implement a registration algorithm (appearance-based approach) to improve the calibration results of the above motion-based approach further.  In this paper, we use the GICP \cite{segal2009generalized} as our registration algorithm. The key benefit of the last step is removing the initialization need for the registration method. Since the objective is non-convex, the algorithm will be stuck in a local minima without a good initial guess. 

\begin{algorithm}
	\caption{Proposed calibration method}
	\begin{algorithmic}[1]
		\REQUIRE Point clouds from $N$ lidars at timestamp $k$: $\mathcal{P}_{k}^{L_i}$.
		\ENSURE Extrinsic parameters from $L_1$ to $L_i$ : $\underset{1\leq i\leq N}{\bigcup}\{(\textbf{R}_{L_i}^{L_1})^{*}, (\textbf{t}_{L_i}^{L_1})^{*}\}$,
		\FOR {each timestamp $k$}
			\STATE $\textbf{R}_{L_i,k}^{L_i,k-1}$, $\textbf{t}_{L_i,k}^{L_i,k-1} \leftarrow $ \textit{motion-estimation}($\mathcal{P}_{k-1}^{L_i}$, $\mathcal{P}_{k}^{L_i}$); 
		\ENDFOR
		\FOR {each lidar $L_{i}$}
			\STATE $\mathcal{T}^{L_i}\leftarrow\underset{1\leq k\leq K}{\bigcup}\{\textbf{R}_{L_i,k}^{L_i,k-1},\textbf{t}_{L_i,k}^{L_i,k-1}\}$;
			\STATE $\mathcal{T}^{L_i}_\textbf{R}\leftarrow\underset{1\leq k\leq K}{\bigcup}\{\textbf{R}_{L_i,k}^{L_i,k-1}\}$;
			\FOR {each loop} 		
				\STATE $(\mathcal{T}^{L_i}_{\textbf{R}})^{'},(\mathcal{T}^{L_i}_{\textbf{R}})^{'}\leftarrow \textit{data-sample}\left(\mathcal{T}^{L_i}_{\textbf{R}}, \mathcal{T}^{L_i}_{\textbf{R}}\right)$;
				\STATE $\textbf{R}_{L_i}^{L_1} \leftarrow \textit{Kabsch}\left[(\mathcal{T}^{L_i}_{\textbf{R}})^{'},(\mathcal{T}^{L_i}_{\textbf{R}})^{'}\right]$;
				\STATE $n_{\text{inlier}} \leftarrow \textit{inlier-number}\left(\mathcal{T}^{L_i}_{\textbf{R}},\mathcal{T}^{L_i}_{\textbf{R}},\textbf{R}_{L_i}^{L_1}\right)$;
			\ENDFOR
			\STATE $\textbf{R}_{L_i}^{L_1} \leftarrow \textit{rotation-with-maximum-inlier}\left(\textbf{R}_{L_i}^{L_1},n_{\text{inlier}}\right)$;
			\FOR {each loop}		
				\STATE $(\mathcal{T}^{L_1})^{'},(\mathcal{T}^{L_i})^{'}\leftarrow \textit{data-sample}\left(\mathcal{T}^{L_1}, \mathcal{T}^{L_i}\right)$;
				\STATE $\textbf{t}_{L_i}^{L_1}\leftarrow \textit{linear-least-square}\left[(\mathcal{T}^{L_1})^{'},(\mathcal{T}^{L_i})^{'},\textbf{R}_{L_i}^{L_1}\right]$;
				\STATE $n_{\text{inlier}}\leftarrow \textit{inlier-number}\left(\mathcal{T}^{L_1},\mathcal{T}^{L_i},\textbf{t}_{L_i}^{L_1}\right)$;
			\ENDFOR		
			\STATE $\textbf{t}_{L_i}^{L_1}\leftarrow \textit{translation-with-maximum-inlier}\left(\textbf{t}_{L_i}^{L_1},n_{\text{inlier}}\right)$;				
			\STATE $(\textbf{R}_{L_i}^{L_1})^{*}, (\textbf{t}_{L_i}^{L_1})^{*} \leftarrow \textit{registration}\left(\mathcal{P}_{K}^{L_1}, \mathcal{P}_{K}^{L_i}, \textbf{R}_{L_i}^{L_1}, \textbf{t}_{L_i}^{L_1}\right)$;
		\ENDFOR
	\end{algorithmic}
	\label{alg.proposed_method}    
\end{algorithm}

\begin{comment}
	Denote the set of relative transformations of lidar $L_1$: 
	$\mathcal{T}^{L_i}$
	=
	$\underset{1\leq k\leq K}{\bigcup}\left\{\textbf{R}_{L_i,k}^{L_i,k-1},\textbf{t}_{L_i,k}^{L_i,k-1}\right\}$,
	$\mathcal{T}^{L_i}_{\textbf{R}}$=$\underset{1\leq k\leq K}{\bigcup}\left\{\textbf{R}_{L_i,k}^{L_i,k-1}\right\}$.
	\\
\end{comment}








==> criticism.tex <==
\section{Criticism of the Existing Work}
\label{criticism}

Determining which approaches are the best is not an easy job. To evaluate a calibration method, various factors should be considered: efficiency, generality, whether or not a calibrated marker is needed. The appearance-based make use of the surrounding information to find data association, but they are restricted to a particular type of sensor pair, like multi-lidar, or lidar-camera. Especially, most of appearance-based approaches can only work on sensors with overlapping fields of view.
On the contrary, motion-based approaches can generally calibrate the multimodal sensor. However, new issues appear because the accuracy of these approaches is highly dependent on the range of motion and the motion estimation of each sensor. Therefore, the system should undergo sufficient motion in structured environments to provide enough data to estimate the rotational and translational offset. 

\subsection{Appearance-Based Approaches}
The selection of the error metric for the ICP algorithm relies on the appearance of surroundings. The point-to-point \cite{besl1992method} is efficient in computation (having a closed-form solution), while the point-to-plane \cite{chen1992object} and the plane-to-plane \cite{segal2009generalized} are less sensitive to noise. The latter two metrics assume that most 3D data points are locally planar and can be described with plane normals. Thus they perform between in structured environments than the point-to-point metric. \\

The minimization of equ. (\ref{equ.icp_pointpoint}) and (\ref{equ.icp_pointplane}) can be optimized via a closed form solution, while in complicated cases like (\ref{equ.icp_planeplane}),  general non-linear least squares algorithms are more effective. In previous work, the Gauss-Newton approach \cite{spek2017joint} or the Levenberg-Marquardt algorithm \cite{fitzgibbon2003robust} have been utilized to minimize the error. However, these gradient-based approaches will converge to a  local minima if the objective is not globally convex. \\

To tackle this problem researchers have resorted other ways to improve the performance of ICP. One solution is to improve the quality of correspondences matching. In these work \cite{he2013pairwise, he2014calibration}, multi-type geometric features are extracted from the 3D maps to build a pair of correspondences.  Another solution is providing a proper initial guess on the extrinsic parameters. In \cite{pandey2017alignment, maroli2017automated}, the ground plane is utilized to align the point clouds in roll, pitch, and Z-axis offset. However, these solutions have strong assumptions on the structures of surroundings.







\subsection{Motion-Based Approaches}
Traditionally, many researchers have focused on finding efficient solutions to equation ($\ref{equ.hand_eye}$). In 1980's, the state-of-the-art solutions were separated into two opposite Directions: coupling and decoupling. The coupling approach operates on global nonlinear optimization, but it time-consuming in a large-scale case. On the contrary, the decoupling approach is more effective and gradually becomes a prominent solution in further years. Tsai et al. \cite{tsai1989new} derived a series of general geometric properties of the hand-eye calibration problem and proposed a  fast and accurate algorithm on the decoupling approach. Later, the computing procedure for rotation was improved in Kabsch's method \cite{kabsch1978discussion}. The Kabsch algorithm performs well even initial guess is not given. This algorithm can find an optimal solution with a minimum least squared error. \\

However, these methods are restricted in indoor environments where the sensors' motion is easily obtained. In more challenging cases, the uncertainty of motion should be considered. Therefore, Taylor et al. \cite{taylor2016motion} combined with appearance-based and motion-based approaches to present a complete calibration system for vehicles. This method is applicable in multimodal sensors and does not require any prior knowledge on the extrinsic parameters. The main contribution of it is building up a probabilistic framework to formulate the uncertainty of sensors' motion. By implementing an appearance-based approach (called Intensity-Motion Metric), the results of lidar-camera calibration are improved. As introduced in Section \ref{sec.overview}, this system consists of three steps: initialization, MLE and refinement. A non-linear least squares technique is utilized in the MLE step. Considering the objective is not convex, the initialization step is necessary to provide an initial guess. Motion-based approaches can be also employed on other platforms. In \cite{heng2013camodocal}, Heng et al. proposed a similar pipeline for multi-camera calibration. The novelty of this method is the usage of bundle adjustment for refinement. However, two limitations are posed in these work: the calibration problem of multi-lidar is still unsolved; they did not explain what a proper motion should look like.











==> experiment_real_data.tex <==
\subsubsection{Experiment Using Real Data}
\label{sec.experiment_read_data}

We calibrated a sensor system which consists of three 16-beam RS-Lidar\footnote{\url{https://www.robosense.ai/rslidar/rs-lidar-16}} on our vehicle [see Fig.\ref{fig.platform}]. As shown in Fig.\ref{fig.sensor_configuration}, lidars are mounted on the front ($L_1$), top ($L_2$), and tail ($L_3$) position respectively to provide wide range observations. We make use of the surrounding buildings and ground as the scan planar surfaces [see Fig.\ref{fig.experiment_planes}].

Two experiments were demonstrated considering two different setups: $L_1$ to $L_2$ as a standard lidar configuration, and $L_1$ to $L_3$ as a challenging lidar configuration. All  lidars were mounted horizontally while $L_3$ was rotated by $180^{\circ}$ in $z\textendash$ axis. 

We take three conventional methods for comparisons. All of them were developed based on the proposed one, but some steps are modified:
\begin{itemize}
	\item Hand-labeling: The planes, their correspondences, and initialization are all given by users directly. 
	\item W/O refinement: The refinement step is removed.
	\item ICP refinement: The nonlinear optimization refinement is replaced by a point-to-plane ICP \cite{pomerleau2013comparing}.
\end{itemize}

Since the ground truth is unavailable, the results provided by the hand-labeling method are considered as the reference values. We randomly selected one frame of measurements for calibration. To make the targeted planar surfaces fully observable, we ensured the vehicle is moved to a proper place.

\begin{table}[]
	\caption{Estimated Extrinsic Parameters from $L_1$ to $L_2$}
	\label{table.estimated_parameters_l1l2}    
	\centering
	\begin{tabular}{ccc}
		\hline \toprule
		\multicolumn{1}{c}{Method}         & \multicolumn{1}{c}{Rotation [rad]} & Error [rad]   \\ \hline
		\multicolumn{1}{c}{Hand-labeling} & \multicolumn{1}{c}{0.0096, 0.0989, 0.0425} & \multicolumn{1}{c}{---}\\
		\multicolumn{1}{c}{w/o refinement} & \multicolumn{1}{c}{-0.0046 -0.1138 -0.0193} & \multicolumn{1}{c}{0.2221}\\             
		\multicolumn{1}{c}{ICP refinement} & \multicolumn{1}{c}{-0.0882, -0.4254, 0.0462} & \multicolumn{1}{c}{0.5333}\\
		\multicolumn{1}{c}{Proposed}       & \multicolumn{1}{c}{0.0012, 0.0892, 0.0276} & \multicolumn{1}{c}{\textbf{0.0203}}\\ \hline \toprule
		\multicolumn{1}{c}{}               & \multicolumn{1}{c}{Translation [m]} & Error [m]  \\ \hline 
		Hand-labeling                     & \multicolumn{1}{c}{0.377002, -0.03309009, -1.23236}       & \multicolumn{1}{c}{---}\\
		w/o refinement                     & \multicolumn{1}{c}{0.314979 0.0509327  -1.23395}       & \multicolumn{1}{c}{0.102694}\\            
		ICP refinement                     & \multicolumn{1}{c}{1.21884 -0.0670357 -1.55964}               & \multicolumn{1}{c}{0.903941}      \\
		Proposed               & \multicolumn{1}{c}{0.336322 0.00271319 -1.19076}   & \multicolumn{1}{c}{\textbf{0.067196}}\\ 
		\hline \toprule
	\end{tabular}
\end{table}

\begin{table}[]
	\caption{Estimated Extrinsic Parameters from $L_1$ to $L_3$}
	\label{table.estimated_parameters_l1l3}    
	\centering
	\begin{tabular}{ccc}
		\hline \toprule
		\multicolumn{1}{c}{Method}         & \multicolumn{1}{c}{Rotation [rad]} & Error [rad] \\ \hline
		\multicolumn{1}{c}{Hand-labeling} & \multicolumn{1}{c}{-0.0161, -0.0192, 3.1392} & \multicolumn{1}{c}{---} \\
		\multicolumn{1}{c}{w/o refinement} & \multicolumn{1}{c}{-0.0527, -0.0212, 3.1328} & \multicolumn{1}{c}{0.0373} \\
		\multicolumn{1}{c}{ICP refinement} & \multicolumn{1}{c}{-0.0333, -0.1329, 3.1277}  & \multicolumn{1}{c}{0.1605} \\
		\multicolumn{1}{c}{Proposed}       & \multicolumn{1}{c}{0.0004, -0.0020, 3.1375}  & \multicolumn{1}{c}{\textbf{0.0238}} \\ \hline \toprule
		\multicolumn{1}{c}{}               & \multicolumn{1}{c}{Translation [m]} &  Error [m]    \\ \hline
		Hand-labeling                     & \multicolumn{1}{c}{-1.96443, 0.04073154, -1.13756}       &  \multicolumn{1}{c}{---} \\
		w/o refinement                     & \multicolumn{1}{c}{-1.92115 0.0968707  -0.80199}          &  \multicolumn{1}{c}{0.341959} \\                
		ICP refinement                     & \multicolumn{1}{c}{-1.95929 0.0473068 -0.383619}          &  \multicolumn{1}{c}{0.753959} \\        
		Proposed               & \multicolumn{1}{c}{-1.9103, 0.052992, -1.0744}           &  \multicolumn{1}{c}{\textbf{0.08357}} \\ 
		\hline \toprule
	\end{tabular}
\end{table}


The results of the proposed method with respect to difference configuration are listed in Table \ref{table.estimated_parameters_l1l2} and \ref{table.estimated_parameters_l1l3}. 
The estimated extrinsic parameters are quite close to hand-labeling method's results. Regarding the relative rotation and translation errors, the proposed method achieved [$0.0203 \text{ rad}, 0.067196 \text{ m}$] and $[0.0238 \text{ rad}, 0.08357\text{ m}]$ on the two configurations respectively. We can also see that larger error was caused by ICP refinement. That is because ICP relies on local correspondences matching, and is thus easily stuck into local minima. On the other hand, the proposed method performs better than that w/o refinement since the nonlinear optimization could further reduce the influence of noise. 
Note that the hand-labeling approach requires human intervention and prior knowledge during calibration process. Hence, the proposed method outperforms hand-labeling approach in terms of efficiency and practicability.

To visualize the calibration results, we transformed the point cloud in $\{L_3\}$ to $\left\{L_1\right\}$ using the estimated parameters provided by the above three methods: W/O refinement, Hand-labeling and Proposed. Top views of the calibrated point clouds are shown in Fig. \ref{fig.fused_point_cloud}. We observe that the point clouds of the hand-labeling and proposed methods have less uncertainty on the planar surfaces. 







==> experiment_simulation.tex <==
\subsubsection{Simulation Using Synthetic Data}
\label{sec.experiment_simulation}

To verify the performance of the proposed algorithm, we randomly generated $9500$ scan points ($7500$ planar points and $2000$ noisy points) in a $10\text{m}\times 10\text{m}\times 10\text{m}$ space. 
The planar points were generated evenly on three planar surfaces, which are subjected to zero-mean Gaussian noise with a standard deviation of $0.1$ m. The rotation angles $\alpha$ in z-axis between $\Pi_1$ and $\Pi_2$ were set in intervals of $(60^{\circ}, 120^{\circ})$, while $\Pi_3$ was set on the bottom, which is orthogonal to $\Pi_1$ and $\Pi_2$. 
The noisy points are also subjected to zero-mean Gaussian distribution with a standard deviation of $5$ m. Lidar $L_1$ was placed arbitrarily where all the planes can be observed. Rotation of the relative poses from $\{L_1\}$ to $\{L_2\}$ were randomly generated within $(0^{\circ}, 20^{\circ})$, $(0^{\circ}, 20^{\circ})$, $(0^{\circ}, 360^{\circ})$ in $x\textendash$, $y\textendash$ and $z\textendash$ axis respectively, and translation of that were generated within $(-1.5, 1.5)$ (m) respectively. An example of the generated points and sensor configuration is visualized in Fig. \ref{fig.simulation_setup_1}.
In our experiments, we randomly select two configuration with different $\mathbf{R}$ and $\mathbf{t}$ [see Table \ref{tab.simulation_result} (top)] as the ground truth to compare with the resulting values.


The difference in rotation is measured according to the angle difference between the reference rotation $\mathbf{R}_{\text{ref}}$ and the resulting rotation $\mathbf{R}_{\text{resulting}}$, which is calculated as $e_{r} = \|\log(\mathbf{R}_{\text{ref}}^{}\mathbf{R}_{\text{resulting}}^{-1})^{\vee}\|_{2}$. 
The operator $\varphi = \log(\mathbf{R})^{\vee}$ is defined to associate $\mathbf{R}$ in $\text{SO}(3)$ to its rotation angle $\varphi\in\mathbb{R}^{3}$ in the axis. 
The difference in translation is computed using vector subtraction as $e_{t} = \|\mathbf{t}_{\text{ref}}^{}-\mathbf{t}_{\text{resulting}}^{}\|_{2}$.

For each group of $\mathbf{R}$ and $\mathbf{t}$, we performed 10 trials on the noisy data and computed the mean and standard deviation of the rotation and translation errors. In Fig. \ref{fig.simulation_result}, blue bars and red lines indicate the mean and standard deviation respectively. Detailed calibration results are shown in Table \ref{tab.simulation_result} (bottom). An example of the calibrated point cloud is shown in Fig. \ref{fig.simulation_setup_2}. In summary, we can see that the rotation and translation errors are tiny on synthetic data. This proves that the proposed method can successfully calibrate the extrinsic parameters.

\begin{table}[]
	\centering
	\caption{The ground truth of two testing configurations (Top) and the calibration results (bottom).}
	\label{tab.simulation_result}    
	\begin{tabular}{ccc}
		\hline 
		\toprule
		\multicolumn{1}{c}{Conf.} & \multicolumn{1}{c}{Rotation {[rad]}} & \multicolumn{1}{c}{Translation {[m]}} \\ \hline
		\textbf{1}                           & 2.7337, -0.3946, -0.1809                & 0.8766, 0.4672, 1.0474                   \\
		\textbf{2}                           & -0.5174, 0.1277, 0.1222                 & 1.3785, -1.3929, 1.3020 \\          
		\hline
		\toprule    \\  
	\end{tabular}    
	
	\begin{tabular}{ccccccc}
		\hline 
		\toprule
		\multicolumn{1}{c}{\multirow{2}{*}{Conf.}}    & \multicolumn{2}{c}{\multirow{2}{*}{$\alpha$ [degree]}} & \multicolumn{2}{c}{Rotation Error [rad]}                                    & \multicolumn{2}{l}{Translation Error [m]}                                    \\ \cline{4-5} \cline{5-7}
		\multicolumn{1}{c}{}                          & \multicolumn{2}{c}{}                                                & \multicolumn{1}{c}{mean}   & \multicolumn{1}{c}{std.}    & \multicolumn{1}{c}{mean}   & \multicolumn{1}{c}{std.}    \\ \hline
		
		\multicolumn{1}{c}{\multirow{7}{*}{\textbf{1}}} & \multicolumn{2}{c}{60}                                             & \multicolumn{1}{c}{0.0035} & \multicolumn{1}{c}{0.0035} & \multicolumn{1}{c}{0.0107} & \multicolumn{1}{c}{0.0161} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{70}                                             & \multicolumn{1}{c}{0}      & \multicolumn{1}{c}{0}      & \multicolumn{1}{c}{0.0001} & \multicolumn{1}{c}{0}      \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{80}                                             & \multicolumn{1}{c}{0.0024} & \multicolumn{1}{c}{0.0056} & \multicolumn{1}{c}{0.0045} & \multicolumn{1}{c}{0.0085} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{90}                                             & \multicolumn{1}{c}{0.0016} & \multicolumn{1}{c}{0.0040} & \multicolumn{1}{c}{0.0100} & \multicolumn{1}{c}{0.0243} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{100}                                            & \multicolumn{1}{c}{0.0051} & \multicolumn{1}{c}{0.0107} & \multicolumn{1}{c}{0.0087} & \multicolumn{1}{c}{0.0178} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{110}                                            & \multicolumn{1}{c}{0.0043} & \multicolumn{1}{c}{0.0063} & \multicolumn{1}{c}{0.0097} & \multicolumn{1}{c}{0.0161} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{120}                                            & \multicolumn{1}{c}{0.0018} & \multicolumn{1}{c}{0.0051} & \multicolumn{1}{c}{0.0083} & \multicolumn{1}{c}{0.0243} \\ \hline
		
		\multicolumn{1}{c}{\multirow{7}{*}{\textbf{2}}} & \multicolumn{2}{c}{60}                                             & \multicolumn{1}{c}{0.0096} & \multicolumn{1}{c}{0.0104} & \multicolumn{1}{c}{0.0260} & \multicolumn{1}{c}{0.0349} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{70}                                             & \multicolumn{1}{c}{0.0036} & \multicolumn{1}{c}{0.0083} & \multicolumn{1}{c}{0.0101} & \multicolumn{1}{c}{0.0274} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{80}                                             & \multicolumn{1}{c}{0.0021} & \multicolumn{1}{c}{0.0064} & \multicolumn{1}{c}{0.0039} & \multicolumn{1}{c}{0.0109} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{90}                                             & \multicolumn{1}{c}{0.0366} & \multicolumn{1}{c}{0.1005} & \multicolumn{1}{c}{0.2245} & \multicolumn{1}{c}{0.6392} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{100}                                            & \multicolumn{1}{c}{0.0126} & \multicolumn{1}{c}{0.0170} & \multicolumn{1}{c}{0.0245} & \multicolumn{1}{c}{0.0339} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{110}                                            & \multicolumn{1}{c}{0.0029} & \multicolumn{1}{c}{0.0057} & \multicolumn{1}{c}{0.0084} & \multicolumn{1}{c}{0.0163} \\ 
		\multicolumn{1}{c}{}                        & \multicolumn{2}{c}{120}                                            & \multicolumn{1}{c}{0.0097} & \multicolumn{1}{c}{0.0139} & \multicolumn{1}{c}{0.0217} & \multicolumn{1}{c}{0.0352} \\ 
		\hline \toprule
	\end{tabular}
\end{table}

==> preliminary.tex <==
 

==> preliminary_idea.tex <==
\section{Preliminary Ideas} 
The problem addressed in this paper is to estimate the extrinsic calibration parameters between 3D lidars \footnote{\url{https://velodynelidar.com/vlp-16.html}}  which are mounted on a vehicle. To make it simple, we make the following assumptions:
\begin{enumerate}
	\item The lidars data are synchronized;
	\item The motion of lidars are known, which can be represented by different types, such as a $4\times 4$ transformation matrix in Euclidean space;
	\item The lidars undergo a series of nondegenerate transformation;	
	\item The lidars are rigid mounting;
	\item The number of lidars $N=2$.
\end{enumerate}

\begin{comment}
\begin{figure}[]
	\centering
	\includegraphics[height=0.2\textwidth]{image/introduction/lidar-crop.pdf}%
	\caption{3D lidar}		
	\label{fig.lidar}
\end{figure}
\end{comment}	

Let us give some notations as follows:
\begin{equation}
	\begin{split}
		\textbf{T}_{y}^{x} \in \mathbb{R}^{4\times4} :& \text{ The transfomation from the frame of sensor }x\text{ to the frame of sensor }y \\
		\textbf{T}_{o,j}^{o,i} \in \mathbb{R}^{4\times4}:& \text{ The transfomation from the odometry frame } \text{ at timestep } i \text{ to the odometry}\\
		&\text{ frame at timestamp } j\\	
		L_1, L_2, \dots L_N :& \text{ The lidar. } \text{In this paper, the frame of } L_1 \text{ is considered as the odometry frame}
	\end{split}
\end{equation}

With assumptions and notations made, our calibration problem can be defined as a extended version of the standard hand-eye calibration problem: Given a sequence of lidar transformations $\textbf{T}_{L_i,k}^{L_i,k-1}, k \in \left\{0, 1,\dots, K\right\}$, compute the relative transformation from the frame of $L_1$ to the frame of other lidars $\textbf{T}_{L_i}^{L_1}$.

Fig.\ref{fig.hand_eye_calibration_vehicle} shows a depiction of how each sensors' motion and relative position are related on a vehicle. As the vehicle moves, $\textbf{T}_{L_i}^{L_1}$ can be recovered by using the transformations at each timestamp:
\begin{equation}
	\textbf{T}_{L_1,k}^{L_1,k-1}\textbf{T}_{L_i}^{L_1} = \textbf{T}_{L_i}^{L_1}\textbf{T}_{L_i,k}^{L_i,k-1}
\end{equation}

\begin{figure}[]
	\centering
	\includegraphics[height=0.3\textwidth]{image/introduction/hand_eye_calibration_vehicle-crop.pdf}
	\caption{The transformation of the lidars on a vehicle at timestamp $k$}		
	\label{fig.hand_eye_calibration_vehicle}
\end{figure}

The equ.(\ref{equ.hand_eye}) can be written into two equations by decomposing
$\textbf{T} = 
\begin{bmatrix}
	\textbf{R} & \textbf{t} \\
	\textbf{0} & 1 \\
\end{bmatrix}$,
\begin{align} 
	\textbf{R}_{L_1,k}^{L_1,k-1}\textbf{R}_{L_i}^{L_1} &=
	\textbf{R}_{L_i}^{L_1}\textbf{R}_{L_i,k}^{L_i,k-1} \label{equ.hand_eye_1} \\
	\textbf{R}_{L_i}^{L_1}\textbf{t}_{L_1,k}^{L_1,k-1} + \textbf{t}_{L_i}^{L_1} &= 
	\textbf{R}_{L_i,k}^{L_i,k-1}\textbf{t}_{L_i}^{L_1} + \textbf{t}_{L_i,k}^{L_i,k-1} \label{equ.hand_eye_2} 
\end{align}

where $\textbf{R} \in \mathbb{R}^{3\times3}$ are the rotation matrices and $\textbf{t} \in \mathbb{R}^{3}$ are the translation vectors. Specifically, $\textbf{R}$ are square and orthogonal with such special properties $\textbf{R}^{T}\textbf{R} = \textbf{I}$ and $\det\textbf{R}=\textbf{I}$.

By combining equ.(\ref{equ.hand_eye_1}) with (\ref{equ.hand_eye_2}), we can write down an optimization problem with an equality constraint on $\textbf{R}_{L_2}^{L_1}$:
\begin{equation}
	\label{equ.optimization}
	\begin{split}
		\underset{\textbf{R}_{L_2}^{L_1}, \textbf{t}_{L_2}^{L_1}}{\text{minimize }} 
		& 
		\sum_{k=2}^{K}
		\left(
		\textbf{R}_{L_1,k}^{L_1,k-1}\textbf{R}_{L_i}^{L_1} -		\textbf{R}_{L_i}^{L_1}\textbf{R}_{L_i,k}^{L_i,k-1}
		\right)\\
		+
		&
		\sum_{k=2}^{K}		
		\left[\left(\textbf{R}_{L_2,k}^{L_2,k-1}-\textbf{I}\right)\textbf{t}_{L_2}^{L_1} 
		+ \textbf{t}_{L_2,k}^{L_2,k-1}- \textbf{R}_{L_2}^{L_1}\textbf{t}_{L_1,k}^{L_1,k-1}\right]\\
		\text{subject to } &\left(\textbf{R}_{L_2}^{L_1}\right)^{T}\textbf{R}_{L_2}^{L_1} = \textbf{I} \\
		&
		\det\textbf{R}_{L_2}^{L_1} =\textbf{I}
	\end{split}	
\end{equation}

This optimization problem has been solved in previous works \cite{taylor2016motion}, \cite{heng2013camodocal}. Considering $\textbf{t}_{L_2}^{L_1}$ is unconstrained, $\textbf{R}_{L_2}^{L_1}$ can be firstly optimized by minimizing the first term of the objective. Based on these works, this paper will present the following contributions:
\begin{enumerate}
	\item I will take the advantages of Lie ground and algebra to solve the problem (6).
	\item I will do experiments on different sensor motions.
	\item I will compare the proposed method with previous works in time complexity with numerical results.
\end{enumerate}



==> result.tex <==
\section{Numerical Results} 
\label{sec.result}
In this section, we demonstrate the accuracy of proposed extrinsic calibration. All experiments are presented with simulated datasets \footnote{\url{https://www.osrfoundation.org/simulated-car-demo/}}.

\subsection{Experimental Setup}
The simulation software is built using ROS Kinetic \cite{quigley2009ros} and Gazebo 8 \cite{koenig2004design}, which contains a simulated vehicle and roads (Fig.\ref{fig.simulation}). This vehicle is equipped with different sensors including 2D and 3D lidars, ultrasonic sensors, cameras. We select this system as it can provide synchronized sensor data and motion's ground truth. In experiments, we focus on three lidars calibration, i.e., $N=3$. 
These lidars are mounted on the front, roof, and back position respectively (Fig.\ref{fig.simulated_vehicle}), which can provide a wide range of observations with a little blind zone. The data output frequency of three lidars is at 10 Hz. 

\begin{figure}[h!]
	\centering
	\begin{minipage}[t]{0.4\textwidth}
		\centering
		\includegraphics[height=0.5\textwidth]{image/introduction/simulation-crop.pdf}
		\caption{A screenshot of the simulation software.}
		\label{fig.simulation}                
	\end{minipage} \hspace{1cm}  
	\begin{minipage}[t]{0.4\textwidth}
		\centering
		\includegraphics[height=0.5\textwidth]{image/introduction/simulated_vehicle-crop.pdf}
		\caption{A figure shows the coordinate systems of three lidars.}
		\label{fig.simulated_vehicle}                
	\end{minipage} 
\end{figure}

\subsection{Extrinsic Calibration Results}
We evaluate the proposed method using different datasets. Datasets are collected by driving the vehicle along with 4 different trajectories which contain synchronized point clouds (perceived by three lidars) and ground truth (lidars' motion and extrinsic parameters). Fig. \ref{fig.trajectory} shows the movements of the vehicle in the world coordinate. Each trajectory lasts from x seconds. The extrinsic parameters from $L_1$ to other lidars we set are shown in Table \ref{tab.extrainsic_parameters}.  $100$ trials are conducted for each trajectory. The calibration results are shown in Fig. \ref{fig.result_box_plot}. Our algorithm can successfully calibrate the rotational and translational offset in the first three trajectories with low absolute error, but fail in the past trajectories. The failure reason is that the last trajectory does not contain enough turns. As Section \ref{subsubsec.initialization} states, the accuracy of rotation and translation estimates is sensitive to the degeneracy of motion.

\begin{figure}[h!]
	\centering
	\includegraphics[height=0.28\textwidth]{image/introduction/trajectory-crop.pdf}
	\caption{Trajectories 1-4 (left to right) of vehicle's movement in the world coordinate system. Each trajectory performs different numbers of tight turns over an uneven surface.}            
	\label{fig.trajectory}
\end{figure}

\begin{table}[]
	\centering
	\caption{The ground truth of extrinsic parameters from $L_1$ to other lidars.}
	\begin{tabular}{|r|r|r|}
		\hline
		Lidar  & $L_2$ & $L_3$\\ \hline
		x [m] & $2.2$ &  $-2$ \\ 
		y [m] & $0$ &  $-2$ \\
		z [m] & $-0.8$ &  $-1$ \\
		roll [rad] & $0$ &  $0$ \\
		pitch [rad] & $0$ &  $0$ \\
		yaw [rad] & $0$ &  $\pi$ \\ \hline
	\end{tabular}
	\label{tab.extrainsic_parameters}
\end{table}

\begin{figure}[]
	\centering
	\caption{Box plots of the error in rotation in rad and translation in meters for optimization with different motion. Each experiment is repeated 100 times.}        
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $1$.]{        
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_1_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage}
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $1$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_1_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}     
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $2$.]{            
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $2$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}     
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}         
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $4$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}             
	\label{fig.result_box_plot}
\end{figure}






